In-N-Out Generative Learning for Dense Unsupervised Video Segmentation

In this paper, we focus on unsupervised learning for Video Object Segmentation (VOS) which learns visual correspondence (i.e., the similarity between pixel-level features) from unlabeled videos. Previous methods are mainly based on the contrastive learning paradigm, which optimize either in image level or pixel level. Image-level optimization (e.g., the spatially pooled feature of ResNet) learns robust high-level semantics but is sub-optimal since the pixel-level features are optimized implicitly. By contrast, pixel-level optimization is more explicit, however, it is sensitive to the visual quality of training data and is not robust to object deformation. To complementarily perform these two levels of optimization in a unified framework, we propose the In-aNd-Out (INO) generative learning from a purely generative perspective with the help of naturally designed class tokens and patch tokens in Vision Transformer (ViT). Specifically, for image-level optimization, we force the out-view imagination from local to global views on class tokens, which helps capture high-level semantics, and we name it as out-generative learning. As to pixel-level optimization, we perform in-view masked image modeling on patch tokens, which recovers the corrupted parts of an image via inferring its fine-grained structure, and we term it as in-generative learning. To discover the temporal information better, we additionally force the inter-frame consistency from both feature and affinity matrix levels. Extensive experiments on DAVIS-2017 val and YouTube-VOS 2018 val show that our INO outperforms previous state-of-the-art methods by significant margins. Code is available: https://github.com/pansanity666/INO_VOS

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/ALL_badcase.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{./figure/Badcase.pdf}
% \DeclaregraphicsExtensions
\vspace{-4mm}
\caption{\textbf{Failure cases on DAVIS-2017 \texttt{val} (upper) and  YouTube-VOS 2018 \texttt{val} (bottom).} 
}
\vspace{-4mm}
\label{fig_all_badcase}
\end{figure}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/Ablation.tex <==
\begin{figure}[t]
\small
\centering
% \vspace{-6mm}
% \includegraphics[width=0.8\linewidth]{./figure/ablation_noPE_short_2.pdf}
% \includegraphics[width=0.9\linewidth]{./figure/Ablation_short_noPE_.pdf}
\includegraphics[width=0.9\linewidth]{./figure/Ablation_short_noPE_.pdf}
% \vspace{-2mm}
\caption{\textbf{Ablation study of training parameters.} We report the \JFm  score evaluated on DAVIS-2017 \texttt{val}. Our baseline configuration (the centered one) is: $M=8,L=4,\tau_{t}=0.04,s=0.8$. }
\label{fig_ablation}
% \vspace{-8mm}
\vspace{-2mm}
\end{figure}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/DAVIS_VIS.tex <==
\begin{figure*}[t]
\centering
% \includegraphics[width=0.70\linewidth]{./figure/DAVIS_vis_2.pdf}
% \includegraphics[width=0.58\linewidth]{./figure/DAVIS_vis_2.pdf}
\includegraphics[width=\linewidth]{./figure/DAVIS_vis_hori.pdf}
% \DeclaregraphicsExtensions
\vspace{-2mm}
\caption{\textbf{Qualitative comparisons on DAVIS-2017 \texttt{val}.} 
We also display the examples of DUL \cite{Dense_araslanov2021dense} and CRW \cite{VRW_jabri2020space}. 
The frame number is illustrated in the upper-right corner.
We mark the salient parts where our method performs better with red dotted boxes. 
% Our INO is more robust to the deformation and can successfully recognize the unseen parts in the given label due to the rich semantic information learnable by in- and out-generative learning.
}
\vspace{-3mm}
\label{fig_DAVIS_vis}
\end{figure*}







==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/DAVIS_VIS_sup.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figure/DAVIS_vis_sup_INOonly.pdf}
% \DeclaregraphicsExtensions
\vspace{-4mm}
\caption{\textbf{Supplemented visualization examples of our INO on DAVIS-2017 \texttt{val}.} 
}
\vspace{-3mm}
\label{fig_DAVIS_vis_sup}
\end{figure*}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/DAVIS_badcase.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figure/DAVIS_badcase.pdf}
% \DeclaregraphicsExtensions
\vspace{-4mm}
\caption{\textbf{Failure cases on DAVIS-2017 \texttt{val}.} 
}
% \vspace{-3mm}
\label{fig_DAVIS_badcase}
\end{figure*}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/YTVOS_VIS.tex <==
\begin{figure*}[t]
\centering
% \includegraphics[width=0.75\linewidth]{./figure/YTVOS_vis_1.pdf}
% \includegraphics[width=0.70\linewidth]{./figure/YTVOS_vis_1.pdf}
\includegraphics[width=\linewidth]{./figure/YTVOS_vis_hori.pdf}
% \DeclaregraphicsExtensions
\vspace{-2mm}
\caption{\textbf{Qualitative comparisons on YouTube-VOS 2018 \texttt{val}}.
Notably, in the second ``hat-trick'' case, we illustrate a hard scenario where the hat is rapidly moving with highly blurry. CRW \cite{VRW_jabri2020space} lost the hat gradually, while DUL \cite{Dense_araslanov2021dense} mistracks toward the human face. Only our INO succeeds to track the hat in motion, which shows that our method can precisely capture the fine-grained correspondence.}
\label{fig_YTVOS_vis}
\vspace{-1mm}
\end{figure*}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/YTVOS_VIS_sup.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figure/YTVOS_vis_sup_INOonly_withegle.pdf}
% \DeclaregraphicsExtensions
\vspace{-4mm}
\caption{\textbf{Supplemented visualization examples of our INO on YouTube-VOS 2018 \texttt{val}.} 
}
% \vspace{-3mm}
\label{fig_YTVOS_vis_sup}
\end{figure*}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/YTVOS_badcase.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figure/YTVOS_badcase.pdf}
% \DeclaregraphicsExtensions
\vspace{-4mm}
\caption{\textbf{Failure cases on YouTube-VOS 2018 \texttt{val}.} 
}
\vspace{-3mm}
\label{fig_YTVOS_badcase}
\end{figure*}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/intro.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=4.8in]{./figure/intro.pdf}
\DeclaregraphicsExtensions
\caption{ \textbf{}  }
\label{fig_intro}
\end{figure}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/figure/sup_ablation.tex <==
\begin{figure}[h]
\small
\centering
% \vspace{-6mm}
% \includegraphics[width=0.8\linewidth]{./figure/ablation_noPE_short_2.pdf}
\includegraphics[width=0.8\linewidth]{./figure/supp_ablation.pdf}
% \vspace{-2mm}
\caption{\textbf{Additional ablation studies of training parameters.}  We report the \JFm  score evaluated on DAVIS-2017 \texttt{val}. Our baseline configuration (the centered one) is: $m=0.996, k=4096, N_l=3, r_h=0.5, PE=64$. }
\label{fig_sup_ablation}
% \vspace{-8mm}
\vspace{-2mm}
\end{figure}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/section/0_abstract.tex <==
% a short version of introduction
% ===== backup =====
% In this paper, we focus on the unsupervised Video Object Segmentation (VOS) which learns visual correspondence from unlabeled videos.
% Previous methods are mainly based on the contrastive learning paradigm, which optimize either in pixel level or image level and show unsatisfactory scalability. Image-level optimization learns pixel-wise information implicitly therefore is sub-optimal for such dense prediction task, while pixel-level optimization ignores the high-level semantic scope for capturing object deformation. To complementarily learn these two levels of information in an unified framework, we propose the In-aNd-Out (INO) generative learning from a purely generative perspective, which captures both high-level and fine-grained semantics by leveraging the structural superiority of Vision Transformer (ViT) and achieves better scalability. Specifically, the in-generative learning recovers the corrupted parts of an image via inferring its fine-grained semantic structure, while the out-generative learning captures high-level semantics by imagining the global information of an image given only random fragments. 
% To better discover the temporal information, we additionally force the inter-frame consistency from both feature level and affinity matrix level.
% Extensive experiments on DAVIS-2017 \texttt{val} and YouTube-VOS 2018 \texttt{val} show that our INO outperforms previous state-of-the-art methods by significant margins.

% ===== v1 =====
In this paper, we focus on unsupervised learning for Video Object Segmentation (VOS) which learns visual correspondence (\textit{i.e.}, the similarity between pixel-level features) from unlabeled videos.
Previous methods are mainly based on the contrastive learning paradigm, which optimize either in image level or pixel level. Image-level optimization (\textit{e.g.}, the spatially pooled feature of ResNet) learns robust high-level semantics but is sub-optimal since the pixel-level features are optimized implicitly. By contrast, pixel-level optimization is more explicit, however, it is sensitive to the visual quality of training data and is not robust to object deformation. 
To complementarily perform these two levels of optimization in a unified framework, we propose the In-aNd-Out (INO) generative learning from a purely generative perspective with the help of naturally designed class tokens and patch tokens in Vision Transformer (ViT).
Specifically, for image-level optimization, we force the out-view imagination from local to global views on class tokens, which helps capture high-level semantics, and we name it as out-generative learning. As to pixel-level optimization, we perform in-view masked image modeling on patch tokens, which recovers the corrupted parts of an image via inferring its fine-grained structure, and we term it as in-generative learning. 
To discover the temporal information better, we additionally force the inter-frame consistency from both feature and affinity matrix levels.
Extensive experiments on DAVIS-2017 \texttt{val} and YouTube-VOS 2018 \texttt{val} show that our INO outperforms previous state-of-the-art methods by significant margins. Code:
\textcolor{red}{\url{https://github.com/pansanity666/INO_VOS}}

==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/section/1_introduction.tex <==


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{figure}[t]
\small
\centering
\includegraphics[width=0.9\linewidth]{./figure/idea-illustration.pdf}
\vspace{-3mm}
\caption{Idea illustration for In-N-Out generative learning. In-generative learning is the in-view recovery of masked patches, while out-generative learning is the out-view imagination from local to global views.}
\label{fig:idea-illustration}
\vspace{-4mm}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

Video Object Segmentation~\cite{R4_added5_wang2021survey, Dense_araslanov2021dense,VOS1_miao2020memory,STM_oh2019video, CFBI_eccv_yang2020collaborative,R2_added0_yang2019unsupervised} (VOS) is a fundamental video understanding task having a wide range of real-world applications, \textit{e.g.}, augmented reality~\cite{VR_xiong2021augmented}, and video editing~\cite{Video_editing_lin2021automated}.
In this task, we aim to segment a specified object instance throughout the entire video sequence, given only the ground-truth object mask on the first frame.
Although the development of convolutional neural networks (CNNs)~\cite{ResNet_he2016deep} has significantly advanced the VOS task, the success of these approaches highly relies on the cost-intensive and time-consuming dense mask annotations to train the networks.
Moreover, the fully-supervised VOS is also largely limited by the diversity and scale of the annotated datasets.
To relieve such limitations, recently unsupervised/self-supervised methods for VOS~\cite{Dense_araslanov2021dense,VRW_jabri2020space,MAST_lai2020mast} have drawn considerable attention, which can completely liberate the request for mask annotations.


However, the previous approaches still suffer from the following perspectives:
(i)\textit{Image-level vs. pixel-level}. Several existing methods~\cite{VRW_jabri2020space,Rethinking_xu2021rethinking} perform self-supervised learning on the image-level features, \textit{e.g.}, the spatially pooled feature of ResNet~\cite{ResNet_he2016deep}. Such optimization can learn robust high-level semantics, however, it is sub-optimal since the pixel-level features used for calculating the final correspondence are learned implicitly. 
Another line of works \cite{Dense_araslanov2021dense,MAST_lai2020mast,TimeCycle_wang2019learning} explicitly optimize on the pixel-level features, however, such paradigm may be sensitive to the visual quality of training data and is lack of the high-level semantic scope which may reduce the robustness toward deformation. We believe that these two levels of optimization are complementary to each other and can be integrated into a unified framework; 
(ii) \textit{CNN vs. ViT}. Previous unsupervised methods~\cite{Dense_araslanov2021dense,VRW_jabri2020space,Rethinking_xu2021rethinking} for VOS adopt the convolutional networks (CNNs)~\cite{ResNet_he2016deep} as the backbone model. However, we propose that  Vision Transformer (ViT)~\cite{ViT_dosovitskiy2020image,DeiT_touvron2021training} is a better choice for unifying these two levels of optimization. Specifically, different from the CNNs which obtain the image-level features via the average pooling of pixel-level features, the naturally designed class tokens and patch tokens of ViT have their own semantic meanings, \textit{i.e.}, class tokens capture the high-level semantics which are suitable for image-level optimization, while patch tokens represent fine-grained details, which are appropriate for pixel-level optimization. 
(iii) \textit{Contrastive vs. generative}. Previous self-supervised methods for VOS~\cite{Dense_araslanov2021dense,VRW_jabri2020space,Rethinking_xu2021rethinking} employ a self-training objective mainly based on contrastive formulation~\cite{MOCO_he2020momentum}. However, their experimental results show unsatisfactory scalability toward the training data scales, especially for the pixel-level methods~\cite{Dense_araslanov2021dense}. 
On the other hand, the recent success of the generative learning paradigm~\cite{MAE_he2021masked} shows its better scalability and robustness. Therefore, we propose that solving the VOS task from the generative learning perspective is promising, yet unexplored.




To tackle the aforementioned issues, we present a simple yet effective framework called In-aNd-Out (INO) generative learning  from a novel fully generative learning perspective.
As opposed to the previous methods~\cite{Dense_araslanov2021dense,VRW_jabri2020space,Rethinking_xu2021rethinking} (detailed in Table \ref{table:method-comparision}), INO integrates image-level and pixel-level optimization in a unified  framework with the help of naturally designed high-level class tokens and fine-grained patch tokens in ViT.


More concretely, as illustrated in Fig.~\ref{fig:idea-illustration}, our INO framework contains two generative objectives, \textit{i.e.}, in-generative learning and out-generative learning. 
(i) \textit{Out-generative learning} is the \textit{out-view} imagination from local views to global views  on class tokens, which corresponds to the image-level optimization. 
We aim to learn high-level visual semantics via imagining the global visual information given only a portion of the local visual part, which may improve the robustness toward deformation and occlusion.
(ii) \textit{In-generative learning} is the \textit{in-view} recovery of randomly masked patch tokens in the feature embedding space, which belongs to the pixel-level optimization. 
The goal of in-generative learning is to capture fine-grained structural information, which is beneficial for recognizing the gradually appearing parts of a semantic object given incomplete labels in the first frame.
In this way, both in-and-out generative objectives complement each other towards better visual representation learning.
To better discover the temporal information, we additionally equip INO with temporally-persistent constraints, by forcing the inter-frame consistency from both feature level and affinity matrix level. Extensive experiments on DAVIS-2017 \texttt{val} and YouTube-VOS 2018 \texttt{val} show that our INO outperforms previous methods by significant margins.
Our main contributions are summarized as follows,
\vspace{-1mm}
\begin{itemize}
\item We propose a simple yet effective framework INO to tackle the challenging unsupervised learning for VOS, which integrates image-level and pixel-level optimization in a unified  framework by leveraging the structural superiority of ViT.
\item To the best of our knowledge, we make the first attempt to conduct unsupervised learning for VOS from a novel fully generative learning perspective  based on the idea of masked image modeling.
\item We attain a new state-of-the-art performance on unsupervised learning for VOS. 
\end{itemize}
\vspace{-2mm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{table/method-comparision}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/section/2_related_work.tex <==

\noindent\textbf{Vision Transformers for Dense Prediction.}
Most previous VOS methods~\cite{Dense_araslanov2021dense,VRW_jabri2020space,MAST_lai2020mast,TimeCycle_wang2019learning,Rethinking_xu2021rethinking} adopt convolutional neural networks (CNNs) as the architectures to learn the visual representations.
Recently, the  development~\cite{ViT_dosovitskiy2020image,DeiT_touvron2021training} of Vision Transformer (ViT) architecture shows overwhelming success over CNNs.
Beyond the simple image classification tasks~\cite{SwinTrans_liu2021swin}, researchers have successfully adopted the ViT architecture in several dense prediction tasks, \textit{e.g.},  object detection~\cite{DERT_carion2020end}, semantic segmentation~\cite{VisTR_wang2021end}, \textit{etc.}
However, these works mainly focus on still images and study the fully-supervised settings.
In contrast, our INO is specially designed to solve the video object segmentation via self-supervised training.
We exploit the architecture privilege of ViT by using the naturally designed high-level class tokens and fine-grained patch tokens. 
%  for image-level and pixel-level optimization, respectively

\noindent\textbf{VOS via Self-supervised Learning.}
Some previous approaches~\cite{VOS2_liang2021rethinking,VOS1_miao2020memory,STM_oh2019video,VOS3_yang2019going,CFBI_yang2021collaborative} learn visual representation fully supervised by annotated datasets with pixel-wise labels.
However, these fully-supervised VOS methods are highly restricted by the diversity of annotated categories and the scale of the annotated dataset.
In this work, we explore a more promising and efficient way which is to leverage self-supervised learning~\cite{DINO_caron2021emerging,MOCO_he2020momentum} to conduct VOS. Previous self-supervised works either only consider the high-level global representations \cite{Rethinking_xu2021rethinking,VRW_jabri2020space}, or directly perform the contrastive learning on the fine-grained pixel-wise features \cite{Dense_araslanov2021dense}. 
Benefiting from the flexibility of vision transformer-based architecture, we optimize both high-level semantics on class tokens and fine-grained semantics on patch tokens, which brings better correspondence learning.

%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
\small
\centering
\includegraphics[width=\textwidth]{./figure/overview_colorized_legend_v2.drawio.pdf}
\caption{\textbf{Overview of INO framework.} For illustration, we assume that the video length $L=2$, and for each frame we crop $1$ global crop and $2$ local crops. 
 (i) \emph{Out-generative learning} is the \emph{out-view} mapping between high-level class tokens, which is composed of $\mathcal{L}_{out \_ g2g}$ and $\mathcal{L}_{out \_ l2g}$. Concisely, $\mathcal{L}_{out \_ g2g}$ is cross-frame calculated between global crop outputs, while $\mathcal{L}_{out \_ l2g}$ is all the possible local-to-global mappings. (ii) \emph{In-generative learning} is the \emph{in-view} recovery on fine-grained patch tokens of global crops, which is composed of $\mathcal{L}_{in \_ mim}$ and  $\mathcal{L}_{in \_ aff}$. In detail, $\mathcal{L}_{in \_ mim}$ is the mapping between mask tokens and the corresponding teacher patch tokens, while $\mathcal{L}_{in \_ aff}$ improves the inter-frame correspondence via bootstrapping.  }
\label{fig_framework}
\vspace{-4mm}
\end{figure*}
%%%%%%%%%%%%%%%%%%%%%

\noindent\textbf{From Contrastive Learning to Generative Learning.}
Recently, contrastive learning~\cite{BYOL_grill2020bootstrap,MOCO_he2020momentum} has been popular for self-supervised learning, which models image similarity and dissimilarity between different views.
Although migrating these methods on VOS tasks~\cite{Dense_araslanov2021dense,VRW_jabri2020space,Rethinking_xu2021rethinking, R3_added3_jeon2021mining, R3_added4_zhao2021modelling} has achieved a preliminary success, the contrastive-based methods strongly depend on data augmentation~\cite{VRW_jabri2020space}, and may also suffer the scalability problem~\cite{Dense_araslanov2021dense,VRW_jabri2020space}.
Inspired by masked language modeling~\cite{BERT_devlin2018bert} in NLP, recent attempts~\cite{BEiT_bao2021beit,MAE_he2021masked} learn representations by masked image modeling.
However, these methods either reconstruct the original images in original pixels~\cite{MAE_he2021masked}, or predict the quantized discrete tokens~\cite{BEiT_bao2021beit}.
As illustrated in Fig.~\ref{fig:idea-illustration}, we discover more abundant supervised signals directly in feature embedding space, by recovering masked patch tokens (in-generative) and imagining global information (out-generative).
To the best of our knowledge, we make the first attempt to address self-supervised learning for VOS from a fully generative learning perspective  based on the idea of masked image modeling.
% \vspace{-2mm}

==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/section/3_method.tex <==

\noindent\textbf{Overview.} Unsupervised learning for video object segmentation targets on achieving semantically discriminative representations via training on unlabeled videos.
During the inference stage, given the mask annotation of the first frame, the label propagation is performed via the correspondence (similarity) between the extracted feature maps \cite{Dense_araslanov2021dense,VRW_jabri2020space,MAST_lai2020mast,Rethinking_xu2021rethinking}.
As illustrated in Fig.~\ref{fig_framework}, we introduce the proposed In-N-Out generative learning framework for the unsupervised learning for VOS, which is composed of out-generative learning on high-level class tokens and in-generative learning on fine-grained patch tokens.
In \S~\ref{sec:framework} we first introduce the generic teacher-student framework.
\S~\ref{sec:out-generative} demonstrates the proposed out-generative learning targets on mining high-level semantic consistency via the imagination between augmented crops. 
\S~\ref{sec:in-generative} introduces the proposed in-generative learning which focuses on achieving fine-grained semantics via the recovery of the corrupted semantic structure.
We \label{sec:pipeline} present the brief training and inference pipeline of the proposed INO in \S~\ref{sec:pipeline}.

% figure of frame pairs
% \begin{figure}[!t]
% \centering
% \includegraphics[width=5.0in]{./figure/frame_pairs.pdf}
% \DeclaregraphicsExtensions
% \caption{ \textbf{The formulation of frame pairs.} Given a video clip of length $L$, it is first split into halves, and the frame pairs are formulated via zipping the two halves. }
% \label{fig_framepairs}
% \end{figure}

% Ori version 
% \subsection{Generative Learning Framework}
% We use the commonly used teacher-student framework \cite{DINO_caron2021emerging,iBOT_zhou2021ibot} for generative learning. The teacher $\mathcal{T}$ and student $\mathcal{S}$ share the same architecture which includes a backbone (e.g, ViT \cite{ViT_dosovitskiy2020image,DeiT_touvron2021training}) and a projection head. A stop-gradient operator is applied on the teacher, and only the student receives gradients. The teacher parameters are the Exponentially Moving Average (EMA) of the student parameters. The teacher output is centered by the computed batch mean \cite{DINO_caron2021emerging}. Then, each network output is normalized with a temperature softmax to get the final categorical distributions  \cite{iBOT_zhou2021ibot}. 
% The output categorical distributions of the teacher are taken as the generation target of the student output and their similarity is measured with a cross entropy loss.

\subsection{Generative Learning Framework}\label{sec:framework}
% We use the commonly used teacher-student framework \cite{DINO_caron2021emerging,iBOT_zhou2021ibot} for generative learning.
% The teacher $\mathcal{T}$ and student $\mathcal{S}$ share the same architecture which includes a backbone (e.g, ViT \cite{ViT_dosovitskiy2020image,DeiT_touvron2021training}) and a projection head. And the teacher parameters are the Exponentially Moving Average (EMA) of the student parameters. Given the student input view $\textbf{s}$ and the teacher input view $\textbf{t}$, we take 
We use the commonly used teacher-student framework \cite{DINO_caron2021emerging,iBOT_zhou2021ibot} for self-supervised learning.
The teacher $\mathcal{T}$ and student $\mathcal{S}$ share the same architecture which includes a backbone (\textit{e.g.}, ViT \cite{ViT_dosovitskiy2020image,DeiT_touvron2021training}) and a projection head.
Without loss of generality, we directly adopt the original ViT implementation.
The improvement of the backbone model is not the focus of this paper.
The teacher parameters are the Exponentially Moving Average (EMA) of the student parameters. To avoid collapse,  a stop-gradient operator is applied to the teacher, and the teacher output is centered by the computed batch mean \cite{DINO_caron2021emerging}. Then, each network outputs (including both class tokens and patch tokens) are normalized with a temperature softmax to get the final categorical distributions  \cite{iBOT_zhou2021ibot}. The output categorical distributions of the teacher are taken as the generation target of the student output and their similarity is measured with a standard cross-entropy loss. 
Notably, the class tokens mainly capture the high-level semantic information, while the patch tokens focus more on the fine-grained details. Therefore, we choose class tokens for out-generative learning and patch tokens for in-generative learning, respectively.

% \vspace{-3.2mm}

\subsection{Out-generative Learning}\label{sec:out-generative}

Given the $i$-th frame in a video clip of length $L$,
we first achieve one global crop $\textbf{g}^{i}$ and $M$ local crops $\{ \textbf{l}^{ij} \}_{j=1}^M$ via \textit{random resized cropping} under different scales.
% \footnote{We use the API from \textit{torchvision.transforms.RandomResizedCrop}.}
Then, \textit{flipping} and \textit{color jitter} are randomly applied for each crop. 
The augmented crops from frames of the same video clip may be quite different in low-level vision due to the performed augmentation and the motion nature of videos.
However, since they are from the same semantic scene, they share similar high-level semantic meaning. 
We intend to leverage such high-level semantic consistency as the supervision signal for out-generative learning, which can be further divided into global-to-global and local-to-global generation, as illustrated in the lower-left part of Fig. \ref{fig_framework}. 

\noindent\textbf{Temporal Consistency via Global-to-global Generation.}
Considering the consecutive nature of video sequences, the global crops from different frames of a certain sequence may share most of the semantic objects when the scale range for cropping is large. In this case, the most salient difference may come from the motion of objects, which should be recognized for better segmentation label propagation, \textit{e.g.}, the person with different poses in different frames should be recognized as the same person. Therefore, we propose to perform generation between these inter-frame global crops to capture such temporal semantic consistency in the presence of motion. 

Specifically, for a sequence of length $L$, we empirically split the sequence into halves and then zip them as frame pairs $ \mathcal{P} = \{(n, L/2 + n ) \}_{n=1}^{L/2}$. Taking $L=6$ as an example, the formulated pairs are $\{ (1,4), (2,5), (3,6) \}$. 
Given a frame pair $(i_{1},i_{2}) \in \mathcal{P} $, all the global crops $\{ \textbf{g}^{i_1}, \textbf{g}^{i_2} \}$ are sent to the student  together with the teacher, and the global-to-global out-generative learning is
performed as:
% \vspace{-6mm}
% \begin{small}
\begin{equation}
\mathcal{L}_{out \_ g2g} = \frac{1}{|\mathcal{P} |} \sum_{(i_1,i_2) \in \mathcal{P}} \sum_{\textbf{t} \in \mathbbm{T}  } \sum_{\textbf{s} \in \mathbbm{S} \backslash \{ \textbf{t} \}  } - \mathcal{T}^{[cls]}(\textbf{t})^{T} log \mathcal{S}^{[cls]}(\textbf{s}),
 \label{eq:out_g2g}
\end{equation}
% \end{small}
where $ \mathbbm{T} = \{ \textbf{g}^{i_1}, \textbf{g}^{i_2} \} $, $ \mathbbm{S} = \{ \textbf{g}^{i_1}, \textbf{g}^{i_2} \}  $.
% and $\mathcal{T}$ and $\mathcal{S}$ represent for the teacher and student module, respectively.

% local to global can provide more aggressive signal
\noindent\textbf{Semantic Correlation via Local-to-global Generation.}
Compared with the global-to-global generation, local-to-global generation solves a harder task, which is to imagine the complete scene given limited information from random semantic fragments. In this scenario, not only motion consistency, but also the inference of the high-level semantic correlation is required.
For example, given the fragment of a motorcross and a part of the human leg, the model is required to infer that ``a rider is riding a motorcross'', as illustrated in Fig. \ref{fig:idea-illustration}. Such high-level inference helps the model to capture more robust and complete semantics, which is beneficial to the stable propagation of masks. 

Specifically, for frame pair $(i_{1},i_{2}) \in \mathcal{P} $, all the local crops are sent to the student and calculated with the previous teacher outputs of global crops. Similar to Eq \ref{eq:out_g2g}, the local-to-global generative learning is performed as:
\begin{equation}
\label{eq:out_l2g}
\mathcal{L}_{out \_ l2g} =   \frac{1}{|\mathcal{P} |} \sum_{(i_1,i_2) \in \mathcal{P}} \sum_{\textbf{t} \in \mathbbm{T}  } \sum_{\textbf{s} \in \mathbbm{S}  } - \mathcal{T}^{[cls]}(\textbf{t})^{T} log \mathcal{S}^{[cls]}(\textbf{s}),
% \label{eq:out}
\end{equation}
where $ \mathbbm{T} = \{ \textbf{g}^{i_1}, \textbf{g}^{i_2} \} $, $ \mathbbm{S} = \{ \textbf{l}^{{i_1}j}, \textbf{l}^{{i_2}j} \}_{j=1}^{M} $.


%%%%%%%%%%%%%%%%%%%%%%%%
\input{table/DAVIS_SOTA}
%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%
\input{table/YTVOS_SOTA}
%%%%%%%%%%%%%%%%%%%%%%%


\subsection{In-generative Learning}
The out-generative learning leverages the class tokens to capture the high-level semantic consistency, however, the dense  segmentation task requires more fine-grained semantic information to precisely capture the correspondence.
Therefore, we introduce the in-generative learning on patch tokens of global crops, which is composed of intra-frame masked image modeling and inter-frame affinity consistency, as shown in the lower-right part of Fig. \ref{fig_framework}. 

% intra-frame MIM
\noindent\textbf{Intra-frame Masked Image Modeling.}\label{sec:in-generative}
Inspired by \cite{BEiT_bao2021beit,iBOT_zhou2021ibot}, we first perform blockwise masking on the input global crops of the \emph{student} module (as illustrated in Fig. \ref{fig_framework}). Specifically, assuming that a global crop from the $i$-th frame $\textbf{g}^i$ is split into $P$ tokens $\textbf{g}^{i} = \{ g_{j}^i \}_{j=1}^P$, we then randomly choose a ratio $r$ as the proportion of masked tokens and get a random mask $ \textbf{m} \in \{0, 1\}^{P}$.
According to $\textbf{m}$, the picked $K = P \cdot r$ tokens $\{ g_{i} | m_i = 1 \}$ are replaced with a global learnable mask token 
% $\textbf{e}_{[msk]}$ 
and get a corrupted token sequence $\hat{\textbf{g}}^i$. After that, $\hat{\textbf{g}}^i$ is sent to the following attention module and prediction head for categorical distributions output. For the \emph{teacher} module, the original unmasked token sequence $\textbf{g}^i$ is kept as input. Finally, similar as Eq. \ref{eq:out_l2g}, we take the corresponding teacher outputs of the masked tokens as the generation target and 
calculate the cross-entropy between them for each global crop in a video clip:

\begin{equation}
\label{eq:in_mim}
\mathcal{L}_{in \_ mim} = \frac{1}{L} \sum_{i=1}^{L} \sum_{j=1}^{P} m_{j} \cdot -\mathcal{T}^{[patch]}_{j}(\textbf{g}^i)^{T} log \mathcal{S}^{[patch]}_{j}(\hat{\textbf{g}}^i) .
\end{equation}

Intuitively, with Eq. \ref{eq:in_mim}, we force the model to generate the corrupted patches based on the limited semantic information from the reserved patches. Such supervision forces the model to achieve the complete and fine-grained semantics, which is important for recognizing the gradually appearing parts given incomplete labels in the first frame. For example, the figure of the person may be incomplete (\textit{i.e.}, corrupted) at the first time of appearance due to the occlusion or limited shooting angle. The model should possess the ability to recognize the rest part of a person which may gradually appear in the following frames, and this is in line with the target of $\mathcal{L}_{in \_ mim}$.




\noindent\textbf{Inter-frame Affinity Consistency.}
$\mathcal{L}_{in \_ mim}$ explores the fine-grained semantic information spatially for each global crop, however, the temporal fine-grained semantic consistency between frames should also be considered, therefore, we propose the affinity consistency constrain as follows. 

Given the $i$-th global crop in a video sequence of length $L$, we represent the $l_2$-normalized $d$-dimensional distribution matrix of the masked tokens from the teacher module  as $Q^i_{t} \in \mathbbm{R}^{K \times d}$. Similarly, the corresponding distribution matrix for the student module is represented as $Q^i_{s} \in \mathbbm{R}^{K \times d}$. Then, the affinity matrix from timestep $i$ to $i+1$ for the teacher outputs is calculated as:
\begin{equation}
\label{eq:affinitymatrix}
A_{t}^{i,i+1} = softmax({(Q^i_t} {Q^{i+1}_t}^T)/ \tau_{t}),
\end{equation}
where $A_{t}^{i,i+1} \in \mathbbm{R}^{K \times K}$ and $\tau_{t}$ is the temperature. Similarly, the corresponding affinity matrix and temperature for the student outputs are $A_{s}^{i,i+1}$ and $\tau_{s}$, respectively. 
Then, we calculate the cross-entropy between these two affinity matrices as follows:
\begin{equation}
\label{eq:in_aff}
\mathcal{L}_{in\_aff} = \frac{1}{L-1} \sum_{i=1}^{L-1} \sum_{j=1}^{K} - {A_{t}^{i,i+1} [j,:]}^T log A_{s}^{i,i+1} [j,:] ,
\end{equation}
where $A_{s}^{i,i+1} [j,:]$ represents for the $j$-th row vector of the matrix,
% intuitive discussion about the affine constrain
% 1. A[j,:] is th correspondence.
% 2. We intendt to improve the correspondence via boostrapping. 
% $\mathcal{L}_{in \_ aff}$ is 
% In Eq. \ref{eq:in_aff}, 
% $A_{s}^{i,i+1} [j,:] \in \mathbbm{R}^{K}$  
which is the softmax normalized cosine similarity between the $j$-th mask token of frame $i$ and all the $K$ masked tokens of frame $i+1$, \textit{i.e.}, the correspondence. Intuitively, we intend to learn the fine-grained temporal correspondence via bootstrapping, which is beneficial for the ultimate goal of propagating segmentation labels. 

% improve such correspondence during via bootstrapping. 

% \subsection{Overall Losses}

% \subsection{Label Propagation}

% Note that $A_{s}^{i,i+1}$ is the correspondence of the output distribution of mask tokens, while $A_{s}^{i,i+1}$ is the correspondence of the corresponding unmasked tokens.





\subsection{Training \& Inference Pipeline}\label{sec:pipeline}
In this subsection, we introduce the whole pipeline for INO to achieve unsupervised learning for VOS.

During the training stage, we start by training the ViT backbone with the raw data from video recognition datasets Kinetics-400 \cite{Kinetics-400_2_kay2017kinetics} and Charades \cite{Charades_sigurdsson2016hollywood} without using any human annotation labels.
Our network is trained in a self-supervised manner with learning objectives:
\begin{equation}
\label{eq:all}
\mathcal{L}_{INO} = \mathcal{L}_{out \_ g2g} + \mathcal{L}_{out \_ l2g} + \mathcal{L}_{in \_ mim} + \mathcal{L}_{in \_ aff} . 
\end{equation}
To maintain simplicity, here we treat all these terms with equal contributions.
Once the backbone model is trained, we can evaluate directly on the DAVIS-2017 \texttt{val}   \cite{DAVIS2017_pont20172017} and YouTube-VOS 2018 \texttt{val} \cite{YouTube-Vos_xu2018youtube} without fine-tuning. 

During inference, the segmentation label of the first frame is provided and then propagated toward the following frames based on the similarity between extracted feature maps. For fair comparison, we use the same label propagation strategy as \cite{Dense_araslanov2021dense,DINO_caron2021emerging,VRW_jabri2020space,Rethinking_xu2021rethinking}, detailed in the supplementary material.

% Specifically, given a  $d$-dimensional feature embedding of the target pixel in current frame, its cosine similarity \textit{w.r.t} the first frame and the $N_c$ previous context frames is calculated. For each frame, restrict attention \cite{MAST_lai2020mast}, which means to only consider the pixels around the target pixel location with a radius of $N_r$, is applied. Then, for all the included reference pixels, the most similar $N_k$ pixels are normalized with a temperature softmax. The final propagated label for the target pixel is the weighted combination of the reference pixel labels.



==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/section/4_experiment.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%
\input{figure/DAVIS_VIS}
%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%
\input{figure/YTVOS_VIS}
%%%%%%%%%%%%%%%%%%%%%%%%


%#################################
\subsection{Experimental Settings}
\textbf{Datasets.}
In order to validate the scalability of the proposed INO, we conduct experiments on two large-scale datasets, including Charades \cite{Charades_sigurdsson2016hollywood} and Kinetics-400 \cite{Kinetics-400_2_kay2017kinetics}. 
Charades \cite{Charades_sigurdsson2016hollywood} dataset spans 9848 videos with an average length of 30s and records the causal everyday activities at home.
Kinetics \cite{Kinetics-400_2_kay2017kinetics} dataset contains significantly more video sequences (around 230K videos with 10s per video on average). 
Note that we directly use raw data from the video dataset, \textit{no} human annotations are involved during the training process.

\noindent\textbf{Evaluation Metrics.}
To verify the generalization ability of INO, we benchmark on two challenging video object segmentation benchmarks: DAVIS-2017 \texttt{val} \cite{DAVIS2017_pont20172017} and YouTube-VOS 2018 \texttt{val} \cite{YouTube-Vos_xu2018youtube}. DAVIS-2017 \texttt{val} contains $30$ videos in 480p, and  YouTube-VOS 2018 \texttt{val} spans 474 videos, and over $90\%$ of them are in 720p. Following previous works~\cite{Dense_araslanov2021dense,Rethinking_xu2021rethinking,VRW_jabri2020space}, we use region similarity ($\mathcal{J}$) and contour accuracy ($\mathcal{F}$) as the evaluation metric \cite{JF_perazzi2016benchmark}.  % see Dense for reference

% \subsubsection{Charades}
% Charades \cite{Charades_sigurdsson2016hollywood} is an action recognition dataset composed of 9,848 videos with an average length of 30 s, showing activities of 267 people who record videos in their own homes, acting out casual everyday activities. The scenes are complicated which may be composed of different combination of furnitures and decoration styles, and the person in a video may move significantly which brings much deformation.

% \subsubsection{Kinetics-400}
% Kinetics-400 \cite{Kinetics-400_carreira2017quo,Kinetics-400_2_kay2017kinetics} is an action recognition dataset which contains around 230K training videos (about 10 s per video) collected from realistic and challenging YouTube
% videos. There are videos with both indoor and outdoor complicated scenes which are in various illumination conditions, and some videos also have large camera motion. Since some of the provided links are expired, we actually use around 195K videos for our unsupervised training.  

% \subsubsection{DAVIS-2017 }
% DAVIS-2017 \cite{DAVIS2017_pont20172017} contains 150 HD videos with over 30K manually labeled instance segmentations. 
% Following previous works \cite{Dense_araslanov2021dense,VRW_jabri2020space,MAST_lai2020mast,Rethinking_xu2021rethinking}, we benchmark on the official semi-supervised video segmentation setting where the ground truth instance segmentation label of the first frame is provided. $30$ videos in 480p are used for this setting. The segmentation results are evaluated with the official released code. 

% \subsubsection{YouTube-VOS 2018}
% YouTube-VOS 2018 \cite{YouTube-Vos_xu2018youtube} is the current largest video segmentation dataset, which has over 4000HD videos of 90 semantic categories. Following \cite{Dense_araslanov2021dense,MAST_lai2020mast,CorrFlow_lai2019self,Colorize_vondrick2018tracking}, we evaluate the semi-supervised setting on YouTube-VOS 2018 \texttt{val} which contains 474 HD videos, and over $90\%$ of them are in 720p. Compared with DAVIA-2017 \texttt{val}, it has larger resolution and more semantic categories. The segmentation results are submitted to an evaluation server \cite{YouTube-Vos_xu2018youtube}.  


\noindent\textbf{Implementation Details.}
% architecture 
    Our INO framework adopts ViT as the backbone model. For fair comparison with the competing methods \cite{Dense_araslanov2021dense,VRW_jabri2020space,Rethinking_xu2021rethinking} that downsample the input resolution for 8 times during inference, we use the ViT-S/8 configuration by default, which possesses comparable parameters as ResNet-50 \cite{ResNet_he2016deep}.  
    For each iteration, we do in-generative learning with a random probability of $0.5$, and $r$ is randomly sampled from a uniform distribution from $0.1$ to $0.5$.
    The temperature is set as $\tau_{s} = 0.1$ and $\tau_{t} = 0.04$, separately.
    The scale range for global and local crops are $(0.05,0.8)$ and $(0.8, 0.95)$, respectively.
    The global crops are resized to $224 \times 224$ while the local crops are resized to $64 \times 64$. The number of local crops $M$ is set as $8$, and the video length $L$ is set as $4$. 
    We train INO for 25 epochs on both Charades and Kinetics-400 with 4 and 8 V100 (16GB) GPUs, respectively.
    Previous works \cite{Dense_araslanov2021dense,VRW_jabri2020space,Rethinking_xu2021rethinking} use the last-block output of ResNet for training, while the middle-block output (\textit{e.g.}, \emph{res 3} block in \cite{VRW_jabri2020space}) for inference. 
    Similarly, we use the output of the last layer (\textit{i.e.}, the $12$-th layer) of ViT for training and empirically use the output of the $7$-th layer for inference.
    More implementation details can be found in the supplementary material. 

%#########################################################
\vspace{-3mm}
\subsection{Quantitative Comparisons with State-of-the-art}

\textbf{Results on DAVIS-2017 benchmark.} 
    In Table \ref{table:DAVIS_with_SOTA}, we report the performance comparisons between our INO and other competing state-of-the-art methods on DAVIS-2017 \texttt{val} benchmark. 
    In a fair comparison where all the methods use the large-scale Kinetics dataset for training, our INO significantly outperforms other state-of-the-art methods by a large margin. 
    For instance, we outperform the second best VFS~\cite{Rethinking_xu2021rethinking} by $3.1\%$ in terms of \JFm ( $72.5\%$ \textit{vs.} $69.4\%$).
    Notably, MAST \cite{MAST_lai2020mast} and CorrFlow \cite{CorrFlow_lai2019self} adopt $2$ times larger image resolution than ours during inference, which leads to larger memory footprint. 
    However, our INO still outperforms MAST~\cite{MAST_lai2020mast} by $7 \%$ on \JFm (72.5\% \textit{vs.} 65.5\%).

\noindent\textbf{Better Scalability.}
Scalability is an important criterion for self-supervised learning methods.
%  Previous methods \cite{Dense_araslanov2021dense,VRW_jabri2020space,MAST_lai2020mast,CorrFlow_lai2019self,ContrastCorr_wang2020contrastive,TimeCycle_wang2019learning,Rethinking_xu2021rethinking} used different training datasets \cite{VLOG_fouhey2018lifestyle,Kinetics-400_2_kay2017kinetics,TrackingNet_Muller_2018_ECCV,OxUvA_valmadre2018long,YouTube-Vos_xu2018youtube}. 
However, as shown in Table~\ref{table:DAVIS_with_SOTA}, the performance of CorrFlow, MAST, and DUL is not positively correlated with the scale of the training dataset. 
And the best performance is not achieved on the largest dataset.
For instance, even though the dataset size is two orders of magnitude smaller ($300k$ \textit{vs.} $4.5k$), the performance of DUL trained with YouTube-VOS is still higher than Kinetics by $0.6 \%$ in \JFm score (68.7 \% \textit{vs.} 69.3 \%). 
%  which is a two orders of magnitude smaller one (300K vs. 4.5K). 
Actually, for such methods, the best performance are achieved on the datasets with higher visual quality and cleaner background, \textit{e.g.}, YouTube-VOS \cite{YouTube-Vos_xu2018youtube}, TrackingNet \cite{TrackingNet_Muller_2018_ECCV}, and OxUvA \cite{OxUvA_valmadre2018long}.
This demonstrates that the previous methods are sensitive to the dataset quality and lack of scalability. 
In contrast, our INO exhibits strong scalability and robustness owing to the generative learning paradigm, \textit{e.g.}, the performance boosts by $5.5$\% from Charades to Kinetics.
% Note that both Charades and Kinetics contain much more noisy background and motion blurry than the rest ones. 



\noindent\textbf{Results on YouTube-VOS 2018 benchmark.} 
Following~\cite{Dense_araslanov2021dense,MAST_lai2020mast}, we additionally evaluate INO on YouTube-VOS 2018 \texttt{val} dataset in Table~\ref{table:YTVOS_with_SOTA}, which is a more challenging benchmark.
% which contains 474 videos with more diversity and is a more comprehensive and challenging test bed than DAVIS-2017 \texttt{val}. 
Our INO reaches a new state-of-the-art which improves over DUL \cite{Dense_araslanov2021dense} by  1.3\% in \Fm  of the ``seen'' category and 0.6\% in mean score.
Compared with CRW \cite{VRW_jabri2020space} which is also trained on Kinetics, our INO outperforms by 1.4\% in the mean score. As to MAST \cite{MAST_lai2020mast} which adopts 2 times larger resolution and a more advanced two-stage inference pipeline, \textit{i.e.}, detecting a ROI first and then considering the correspondence bounded by the ROI, our INO still outperforms by a significant margin ($71.3$\% \textit{vs.} $64.2$\%). 
\vspace{-3mm}

%#################################
\subsection{Qualitative Analysis}
We visualize the mask propagation results in Fig. \ref{fig_DAVIS_vis} and Fig. \ref{fig_YTVOS_vis} for DAVIS-2017 \texttt{val} and YouTube-VOS 2018 \texttt{val}, respectively. 
For better comparison, we also illustrate the results for DUL \cite{Dense_araslanov2021dense} and CRW \cite{VRW_jabri2020space}.
We observe that our INO achieves better qualitative results and is superior in the following aspects:

\noindent\textbf{Robust to Unseen Parts.}
As illustrated in the first ``motorcross-jump'' scenario of Fig. \ref{fig_DAVIS_vis}, the right leg and back view of the rider is unseen in the given label of the first frame.
The contrastive learning based methods CRW \cite{VRW_jabri2020space} and DUL \cite{Dense_araslanov2021dense} fail to track such unseen parts in the following sequences, while our INO tracks them successfully (see frame $15$ and $35$). We attribute this superiority mainly to the in-generative learning objective, which helps capture the complete semantic structure of the corrupted parts. 

\noindent\textbf{Robust to Deformation.} 
% Deformation is also an important obstacle for the mask propagation. 
Our INO shows better robustness to deformation compared with previous methods.
For instance, in the ``motorcross-jump'' scenario of Fig. \ref{fig_DAVIS_vis}, the back wheel deforms significantly during the motion process, while only our INO can consistently identify the entire back wheel. 
The out-generative learning process fully exploits the semantic consistency between deformed objects from different frames during training. 
Intuitively, this supervised signal improves the robustness of features toward the deformation. 

\noindent\textbf{Less Artifacts.}
During the mask propagation process, the label may shift toward the background which shares a similar pattern with the target object, and this is termed as the ``bleeding'' artifacts in \cite{Dense_araslanov2021dense}. 
As illustrated in the first ``motorcycle'' case in Fig. \ref{fig_YTVOS_vis}, both CRW \cite{VRW_jabri2020space}
and DUL \cite{Dense_araslanov2021dense} suffer this issue in frame 65 and 85, while our INO gives a more complete and stable mask even under a noisy background. 

\noindent\textbf{Fine-grained Correspondence.}
In the second ``hat-trick'' case of Fig. \ref{fig_YTVOS_vis}, we illustrate an extremely hard scenario that requires the ability to precisely capture the fine-grained details. Specifically, a small hat in high motion is thrown by the actor. As the label propagates, CRW \cite{VRW_jabri2020space} lost the hat gradually, and DUL \cite{Dense_araslanov2021dense} shifts to the actor's face immediately, while only our INO tracks the hat consistently and precisely. 

%#############################################


%%%%%%%%%%%%%%%%%%%%%
\input{table/Ablation}
%%%%%%%%%%%%%%%%%%%%%


\subsection{Ablation Studies}
\label{sec_ablation_study}
We investigate the effectiveness of learning objectives in Table \ref{table:Ablation}, and the influence of training parameters in Fig. \ref{fig_ablation}. The performance trained on Charades and evaluated on DAVIS-2017 \texttt{val} is reported.

\noindent\textbf{Effectiveness of In-N-Out Generative Learning.}
In Table~\ref{table:Ablation}, we investigate the effectiveness of In-N-Out generative learning objectives. We set the out-generative learning between global crops as the baseline configuration and then add each term gradually.
With only out-generative learning between global crops
($\mathcal{L}_{out \_ g2g}$), the model can achieve 45.6\% in \JFm. 
After adding the out-generative learning between local and global crops ($\mathcal{L}_{out \_ l2g}$), the \JFm score boosts for
8.6\%, which shows that the high-level semantic inference from local to global crops can significantly help to improve the performance.
With out-generative learning only, the model achieves a performance of 54.2\%. 
Notably, the performance is further improved significantly by 11.2\% in \JFm score after including the in-generative learning via masked image modeling ($\mathcal{L}_{in \_ mim}$), which shows the importance of fine-grained structural semantic. Finally, the best performance is achieved after $\mathcal{L}_{in \_ aff}$ is introduced, which improves the temporal correspondence via bootstrapping.

% We illustrate all the experimental results for this section in Fig. \ref{fig_ablation}. 

%%%%%%%%%%%%%%%%%%%%%%%
\input{figure/Ablation}
%%%%%%%%%%%%%%%%%%%%%%%



\noindent\textbf{Temperature of Affinity Constrain.}
In $\mathcal{L}_{in \_ aff}$, we use $\tau_{s}$ and $\tau_{t}$ as the temperature for student and teacher affinity matrix, separately.
We fix the student temperature $\tau_{s}$ as $0.1$ and change $\tau_{t}$ as $\{0.02, 0.04, 0.06\}$, where smaller $\tau_{t}$ gives sharper target distributions. As illustrated by the yellow one in Fig.~\ref{fig_ablation}, $\tau_{t}=0.04$ gives a moderate sharpness and performs best. 

% \vspace{-3mm}
\noindent\textbf{Sequence Length.} 
We increase the sequence length $L$ as $\{2,4,6\}$, and find that $L=4$ performs best, as illustrated by the orange one in Fig. \ref{fig_ablation}. Longer sequence length brings larger difference between the paired frames, however, too much difference (\textit{e.g.}, the object may disappear in the later frames) incurs the mismatch between the source and target views, which increases the training noise.
Therefore, a moderate sequence length ($L=4$) gives the best performance.

\noindent\textbf{Number of Local Crops.} % 
We vary the local crops number $M$ as $\{6, 8, 10 \}$. More local crops bring more radical high-level semantic inference. As illustrated by the green one in Fig. \ref{fig_ablation}, $M=8$ gives the best performance, which is tangibly better than $M=6$ and $M=10$, \textit{e.g.}, $M=10$ leads to a drop in \JFm score by 2.1\%. We infer that too many local crops may lead to overfitting toward the noise, and a moderate $M=8$ is sufficient. 

\noindent\textbf{Scale Threshold for Random Resized Cropping.}
We use the random resized cropping which first samples views with scale range $(0.05, s)$ for local crops and $(s, 0.95)$ for global crops, and then resized them to $64 \times 64$ and $224 \times 224$, respectively. We vary the threshold $s$ as $\{0.4, 0.6, 0.8\}$. Larger $s$ leads to more diverse local crops and more stable global crops containing richer information about the scene. By observing the gray one in Fig. \ref{fig_ablation}, we find that the performance becomes better as $s$ increases from $0.4$ to $0.8$. We infer  that the global crops with rich global information are more helpful to the semantic inference from local to global. 


% \subsection{}
\noindent\textbf{Flipping and Color Jitter.}
\input{table/FC_Ablation}
After obtaining global and local crops via \emph{random resized cropping},  we empirically perform  \emph{flipping} and \emph{color jitter} (F\&C) randomly only for local crops. We investigate  $4$ configurations in Table \ref{table:FC_Ablation}. We observe that operating F\&C on global crops will reduce the performance. For instance, compared with not using F\&C, the \JFm score drops by 3.0\% from 66.6\% to 63.6\% after performing F\&C on global crops. We infer that more stable global crops are preferred for the generation process. Performing F\&C only on local crops provides the best performance on average (67.0\% in \JFm score), therefore we take it as the default configuration. 


\input{figure/ALL_badcase}
\subsection{Limitation}
\label{limitation}
We provide failure cases on DAVIS-2017 \texttt{val} and YouTube-VOS 2018 \texttt{val} in Fig. \ref{fig_all_badcase}. We observe that the performance tends to be unsatisfactory under the following challenging scenarios: (i) \emph{Multiple extremely similar instances.} For instance, the two dogs in case 1 of Fig. \ref{fig_all_badcase} are very similar in low-level vision, therefore the labels are confused during the later time steps. (ii) \emph{Long-term and large-area occlusion.} As illustrated by case 2 of Fig. \ref{fig_all_badcase}, the labels tend to lose the object after the long-term and large-area occlusion.
We can observe that there is still room for improvement in the aforementioned challenging cases. 


% We will make efforts to improve the robustness toward the aforementioned scenarios in future work.

% \input{figure/DAVIS_badcase}
% \input{figure/YTVOS_badcase}

% \subsubsection{Initialized Position Embedding Resolution}
% \subsubsection{Layer Number in Prediction Head}
% \subsubsection{Momentum}

% need table 
% \subsubsection{Influence of Flipping and Color Jitter}

% best illustrated with plot 
% \subsubsection{Inference Layer}



==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/section/5_conclusion.tex <==
In this paper, to tackle the challenging unsupervised learning for VOS, we proposed a simple yet effective framework called In-N-Out (INO) generative learning. 
The proposed INO is a novel fully-generative learning framework via in-view image recovery and out-view image imagination, which integrates both pixel-level and image-level optimization in a unified framework.
Without any annotation data, we effectively learn robust visual representations in a self-supervised manner and achieve the new state-of-the-art performance among unsupervised learning methods for VOS. However, there is still a long way to go considering the analyzed limitations in \S~\ref{limitation}  and the performance gap between the unsupervised and the supervised methods.
% Although INO achieves a large improvement for the unsupervised VOS task, there is still a long way to go. There is still a performance gap between the unsupervised and the supervised methods.
Thus, more effective algorithms are still required to alleviate this gap. 
We hope that our efforts will motivate more researchers and ease future research.

==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/table/Ablation.tex <==
\begin{table}[t]
% \footnotesize
\small
\caption{\textbf{Effectiveness of In-N-Out generative learning objectives.} All results are evaluated on DAVIS-2017 \texttt{val} benchmark. }
\vspace{-3mm}
\begin{center}
 \setlength{\tabcolsep}{3mm}{
\begin{tabular}{l|l|ccccc}
\hline
\rowcolor{LightGray}

                  & \textbf{Objective} & \textbf{\JFm}  & \textbf{\Jm}   & \textbf{\Jr}   & \textbf{\Fm}   & \textbf{\Fr}   \\ \hline
\multirow{2}{*}{\rotatebox{90}{Out}} & $\mathcal{L}_{out \_ g2g}$          & 45.6          & 43.4          & 46.3          & 47.7          & 54.8          \\
                  & $+\mathcal{L}_{out \_ l2g}$        & 54.2          & 51.0          & 56.1          & 57.4          & 64.0          \\ \hline
\multirow{2}{*}{\rotatebox{90}{In}} & $+\mathcal{L}_{in \_ mim}$          & 65.4          & 62.4          & 71.6          & 68.3          & 80.1          \\
                  & $+\mathcal{L}_{in \_ aff}$           & \textbf{67.0} & \textbf{63.7} & \textbf{72.7} & \textbf{70.4} & \textbf{82.9} \\ \hline
\end{tabular}}
\end{center}
\label{table:Ablation}
\vspace{-4mm}
\end{table}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/table/Backbone_Ablation.tex <==
\begin{table}[h]
% \footnotesize
\small
\caption{Influence of backbone architectures. All results are evaluated on DAVIS-2017 \texttt{val} benchmark. }
\vspace{-1mm}
\begin{center}
 \setlength{\tabcolsep}{3.9mm}{
\begin{tabular}{l|ccccc}
\hline
\rowcolor{LightGray}
\textbf{Arch} & \JFm            & \Jm             & \Jr             & \Fm             & \Fr             \\ \hline
ViT-T/8       & 65.7          & 62.8          & \textbf{73.0} & 68.7          & 81.6          \\ 
ViT-S/8       & \textbf{67.0} & \textbf{63.7} & 72.7          & \textbf{70.4} & \textbf{82.9} \\ \hline
\end{tabular}}
\end{center}
\label{table:Backbone_Ablation}
\vspace{-1mm}
\end{table}

==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/table/DAVIS_SOTA.tex <==
\begin{table*}[t]
% \footnotesize
\small
\caption{\textbf{Comparisons with state-of-the-art methods on DAVIS-2017 \texttt{val}.} RN-18 and ViT-S/8 represent for ResNet-18 and Vit-Small with a patch size of 8, separately. ``\dag'' means using 2 times larger resolution for inference. We also report the number of video sequences (N) and the total video duration (T) for each dataset.  }
\vspace{-2mm}
\begin{center}
 \setlength{\tabcolsep}{5.2mm}{
\begin{tabular}{l|ccc|ccccc}
\rowcolor{LightGray}
\hline
\textbf{Method}       & \textbf{Arch} & \textbf{Dataset} & \textbf{N/T} & \textbf{\JFm}  & \textbf{\Jm}   & \textbf{\Jr}   & \textbf{\Fm}   & \textbf{\Fr}   \\ \hline \hline
TimeCycle \cite{TimeCycle_wang2019learning}    & RN-18                     & VLOG                  & 114K / 344h  & -             & 40.1          & -             & 38.3          & -             \\
TimeCycle \cite{TimeCycle_wang2019learning}    & RN-50                     & VLOG                  & 114K / 344h  & -             & 41.9          & -             & 39.4          & -             \\ \hline
CorrFlow\dag \cite{CorrFlow_lai2019self}     & RN-18                     & Kinetics              & 300K / 833h  & 49.5          & 47.7          & 53.2          & 51.3          & 56.5          \\
CorrFlow\dag \cite{CorrFlow_lai2019self}     & RN-18                     & OxUvA                & 366 / 14h    & 50.3          & 48.4          & 53.2          & 52.2          & 56.0          \\ \hline
ContCorr \cite{ContrastCorr_wang2020contrastive} & RN-18                       & TrackingNet           & 30K / 140h   & 63.0          & 60.5          & -             & 65.5          & -             \\ \hline
MAST\dag \cite{MAST_lai2020mast}         & RN-18                  & OxUvA                 & 366 / 14h    & 63.7          & 61.2          & 73.2          & 66.3          & 78.3          \\
MAST\dag \cite{MAST_lai2020mast}         & RN-18                  & YT-VOS                & 4.5K / 5h    & 65.5          & 63.3          & 73.2          & 67.6          & 77.7          \\ \hline
CRW \cite{VRW_jabri2020space}          & RN-18                   & Kinetics              & 300K / 833h  & 67.6          & 64.8          & 76.1          & 70.2          & 82.1          \\ \hline
JSTG \cite{R3_added4_zhao2021modelling}  & RN-18                   & Kinetics              & 300K / 833h  & 68.7          & 65.8          & 77.7           & 71.6          & 84.3          \\ \hline
DUL \cite{Dense_araslanov2021dense}          & RN-18                    & OxUvA               & 366 / 14h    & 65.3          & 63.4          & 76.1          & 67.2          & 79.7          \\
DUL \cite{Dense_araslanov2021dense}          & RN-18                    & Kinetics              & 300K / 833h  & 68.7          & 66.7          & 81.4          & 70.7          & 84.1          \\
DUL \cite{Dense_araslanov2021dense}          & RN-18                       & YT-VOS                & 4.5K / 5h    & 69.3          & 67.1          & 81.2          & 71.6          & 84.9          \\
DUL \cite{Dense_araslanov2021dense}          & RN-18                    & TrackingNet           & 30K / 140h   & 69.4          & 67.1          & 80.9          & 71.7          & 84.8          \\ \hline
VFS \cite{Rethinking_xu2021rethinking}          & RN-18                  & Kinetics              & 300K / 833h  & 67.6          & 64.8          & -             & 70.2          & -             \\
VFS \cite{Rethinking_xu2021rethinking}          & RN-50                 & Kinetics              & 300K / 833h  & 69.4          & 66.7          & -             & 72.0          & -             \\ \hline
\textbf{INO (Ours)}    & ViT-S/8                 & Charades              & 10K / 82h    & 67.0          & 63.7          & 72.7          & 70.4          & 82.9          \\
\textbf{INO (Ours)}    & ViT-S/8                 & Kinetics              & 300K / 833h  & \textbf{72.5} & \textbf{68.7} & \textbf{82.0} & \textbf{76.3} & \textbf{89.0} \\ \hline
\end{tabular}}
\end{center}
\label{table:DAVIS_with_SOTA}
\vspace{-4mm}
\end{table*}




% no backbone version
% \begin{tabular}{lcccccccc}
% \hline
% \textbf{Method}       & \textbf{x2} & \textbf{Data} & \textbf{n/t}         & \textbf{JFm}  & \textbf{Jm}   & \textbf{Jr}   & \textbf{Fm}   & \textbf{Fr}   \\ \hline
% \textbf{TimeCycle}    & \textbf{-}  & \textbf{VLOG}         & \textbf{114K / 344h} & -             & 40.1          & -             & 38.3          & -             \\
% \textbf{TimeCycle}    & -           & VLOG                  & 114K / 344h          & -             & 41.9          & -             & 39.4          & -             \\ \hline
% \textbf{CorrFlow}     & \checkmark         & Kinetics              & 300K / 833h          & 49.5          & 47.7          & 53.2          & 51.3          & 56.5          \\
% \textbf{CorrFlow}     & \checkmark         & OxUvA                 & 366 / 14h            & 50.3          & 48.4          & 53.2          & 52.2          & 56.0          \\ \hline
% \textbf{ContrastCorr} & -           & TrackingNet           & 30K / 140h           & 63.0          & 60.5          & -             & 65.5          & -             \\ \hline
% \textbf{MAST}         & \checkmark         & OxUvA                 & 366 / 14h            & 63.7          & 61.2          & 73.2          & 66.3          & 78.3          \\
% \textbf{MAST}         & \checkmark         & YT-VOS                & 4.5K / 5h            & 65.5          & 63.3          & 73.2          & 67.6          & 77.7          \\ \hline
% \textbf{CRW}          & -           & Kinetics              & 300K / 833h          & 67.6          & 64.8          & 76.1          & 70.2          & 82.1          \\ \hline
% \textbf{DUL}          & -           & OxUvA                 & 366 / 14h            & 65.3          & 63.4          & 76.1          & 67.2          & 79.7          \\
% \textbf{DUL}          & -           & Kinetics              & 300K / 833h          & 68.7          & 66.7          & 81.4          & 70.7          & 84.1          \\
% \textbf{DUL}          & -           & YT-VOS                & 4.5K / 5h            & 69.3          & 67.1          & 81.2          & 71.6          & 84.9          \\
% \textbf{DUL}          & -           & TrackingNet           & 30K / 140h           & 69.4          & 67.1          & 80.9          & 71.7          & 84.8          \\ \hline
% \textbf{VFS}          & -           & Kinetics              & 300K / 833h          & 67.6          & 64.8          & -             & 70.2          & -             \\
% \textbf{VFS}          & -           & Kinetics              & 300K / 833h          & 69.4          & 66.7          & -             & 72.0          & -             \\ \hline
% \textbf{INO(ours)}    & -           & Charades              & 10K / 82h            & 67.0          & 63.7          & 72.7          & 70.4          & 82.9          \\
% \textbf{INO(ours)}    & -           & Kinetics              & 300K / 833h          & \textbf{72.5} & \textbf{68.7} & \textbf{82.0} & \textbf{76.3} & \textbf{89.0} \\ \hline
% \end{tabular}

% \begin{tabular}{l|cc|cc|ccccc}
% \rowcolor{LightGray}
% \hline
% \textbf{Method}       & \textbf{Arch} & \textbf{$\times 2$} & \textbf{Dataset} & \textbf{N/T} & \textbf{\JFm}  & \textbf{\Jm}   & \textbf{\Jr}   & \textbf{\Fm}   & \textbf{\Fr}   \\ \hline \hline
% TimeCycle \cite{TimeCycle_wang2019learning}    & RN-18             & -           & VLOG                  & 114K / 344h  & -             & 40.1          & -             & 38.3          & -             \\
% TimeCycle \cite{TimeCycle_wang2019learning}    & RN-50             & -           & VLOG                  & 114K / 344h  & -             & 41.9          & -             & 39.4          & -             \\ \hline
% CorrFlow\dag \cite{CorrFlow_lai2019self}     & RN-18             & \checkmark         & Kinetics              & 300K / 833h  & 49.5          & 47.7          & 53.2          & 51.3          & 56.5          \\
% CorrFlow\dag \cite{CorrFlow_lai2019self}     & RN-18             & \checkmark         & OxUvA                & 366 / 14h    & 50.3          & 48.4          & 53.2          & 52.2          & 56.0          \\ \hline
% ContCorr \cite{ContrastCorr_wang2020contrastive} & RN-18             & -           & TrackingNet           & 30K / 140h   & 63.0          & 60.5          & -             & 65.5          & -             \\ \hline
% MAST\dag \cite{MAST_lai2020mast}         & RN-18             & \checkmark         & OxUvA                 & 366 / 14h    & 63.7          & 61.2          & 73.2          & 66.3          & 78.3          \\
% MAST\dag \cite{MAST_lai2020mast}         & RN-18             & \checkmark         & YT-VOS                & 4.5K / 5h    & 65.5          & 63.3          & 73.2          & 67.6          & 77.7          \\ \hline
% CRW \cite{VRW_jabri2020space}          & RN-18             & -           & Kinetics              & 300K / 833h  & 67.6          & 64.8          & 76.1          & 70.2          & 82.1          \\ \hline
% DUL \cite{Dense_araslanov2021dense}          & RN-18             & -           & OxUvA               & 366 / 14h    & 65.3          & 63.4          & 76.1          & 67.2          & 79.7          \\
% DUL \cite{Dense_araslanov2021dense}          & RN-18             & -           & Kinetics              & 300K / 833h  & 68.7          & 66.7          & 81.4          & 70.7          & 84.1          \\
% DUL \cite{Dense_araslanov2021dense}          & RN-18             & -           & YT-VOS                & 4.5K / 5h    & 69.3          & 67.1          & 81.2          & 71.6          & 84.9          \\
% DUL \cite{Dense_araslanov2021dense}          & RN-18             & -           & TrackingNet           & 30K / 140h   & 69.4          & 67.1          & 80.9          & 71.7          & 84.8          \\ \hline
% VFS \cite{Rethinking_xu2021rethinking}          & RN-18             & -           & Kinetics              & 300K / 833h  & 67.6          & 64.8          & -             & 70.2          & -             \\
% VFS \cite{Rethinking_xu2021rethinking}          & RN-50             & -           & Kinetics              & 300K / 833h  & 69.4          & 66.7          & -             & 72.0          & -             \\ \hline
% \textbf{INO (Ours)}    & ViT-S/8            & -           & Charades              & 10K / 82h    & 67.0          & 63.7          & 72.7          & 70.4          & 82.9          \\
% \textbf{INO (Ours)}    & ViT-S/8            & -           & Kinetics              & 300K / 833h  & \textbf{72.5} & \textbf{68.7} & \textbf{82.0} & \textbf{76.3} & \textbf{89.0} \\ \hline
% \end{tabular}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/table/FC_Ablation.tex <==
\begin{table}[t]
% \footnotesize
\small
\caption{Influence of different configurations of operating \emph{flipping} and \emph{color jitter} (F\&C). 
% All results are evaluated on DAVIS-2017 \texttt{val} benchmark. 
}
\vspace{-1mm}
\begin{center}
 \setlength{\tabcolsep}{2mm}{
\begin{tabular}{c|c|c|ccccc}
\hline
\rowcolor{LightGray}
\multicolumn{1}{l|}{\textbf{}} & \multicolumn{1}{l|}{\textbf{Global?}} & \multicolumn{1}{l|}{\textbf{Local?}} & \multicolumn{1}{c}{\JFm}            & \multicolumn{1}{c}{\Jm}             & \multicolumn{1}{c}{\Jr}             & \multicolumn{1}{c}{\Fm}             & \multicolumn{1}{c}{\Fr}             \\ \hline
\multirow{4}{*}{F\&C} & -                            & -                       & \multicolumn{1}{c}{66.6} & \multicolumn{1}{c}{63.5} & \multicolumn{1}{c}{\textbf{74.7}} & \multicolumn{1}{c}{69.7} & \multicolumn{1}{c}{82.4} \\ %\cline{2-8} 
                               & \cmark                                 & -                                    & 63.6                              & 60.8                              & 69.5                              & 66.5                              & 77.9                              \\ %\cline{2-8} 
                               & -                                     & \cmark                                & \textbf{67.0}                     & \textbf{63.7}                     & 72.7                              & \textbf{70.4}                     & \textbf{82.9}                     \\ %\cline{2-8} 
                               & \cmark                                 & \cmark                                & 66.2                              & 63.3                              & 73.3                              & 69.1                              & 82.1                              \\ \hline
\end{tabular}}
\end{center}
\label{table:FC_Ablation}
\vspace{-4mm}
\end{table}

==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/table/YTVOS_SOTA.tex <==
\begin{table}[!t]
% \footnotesize
\small
\caption{ \textbf{Comparisons with state-of-the-art methods on YouTube-VOS 2018 \texttt{val} benchmark}. The object classes in the \texttt{val} set are partly overlapped with the \emph{training} set, therefore the performance is distinguished as ``seen'' and ``unseen'' categories. 
All results are evaluated and reported through the online testing server~\cite{YouTube-Vos_xu2018youtube}.}
\vspace{-2mm}
\begin{center}

% \begin{tabular}{l|ccccccc}
% \hline
% \rowcolor{LightGray}
%  &  &  &  & \multicolumn{2}{c}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} \\\cline{5-8}
% \rowcolor{LightGray}
% \multirow{-2}{*}{\textbf{Method}}                                 &    \multirow{-2}{*}{\textbf{$\times 2$}}                          & \multirow{-2}{*}{\textbf{Dataset}}                               &   \multirow{-2}{*}{\textbf{Mean}}                            & \textbf{\Jm}     & \textbf{\Fm}     & \textbf{\Jm}      & \textbf{\Fm}      \\ \hline \hline
% Colorize \cite{Colorize_vondrick2018tracking}                & -                            & Kinetics                                           & 38.9                           & 43.1            & 38.6            & 36.6             & 37.4             \\ 
% CorrFlow\dag \cite{CorrFlow_lai2019self}                & \checkmark                          & OxUvA                                              & 46.6                           & 50.6            & 46.6            & 43.8             & 45.6             \\ 
% MAST\dag \cite{MAST_lai2020mast}                    & \checkmark                          & YT-VOS                                             & 64.2                           & 63.2            & 64.9            & 60.3             & 67.7             \\ 
% CRW \cite{VRW_jabri2020space}                     & -                            & Kinetics                                           & 69.9                           & 68.7            & 70.2            & 65.4             & 75.2             \\ 
% DUL \cite{Dense_araslanov2021dense}                     & -                            & YT-VOS                                           & 69.9                           & 69.6            & 71.3            & 65.0    & 73.5             \\
% DUL \cite{Dense_araslanov2021dense}                     & -                            & Kinetics                                           & 70.6                           & 69.9            & 71.3            & \textbf{66.5}    & 74.8             \\
% DUL \cite{Dense_araslanov2021dense}                     & -                            & TrackingNet                                        & 70.7                           & 70.2            & 71.9            & 66.3             & 74.5             \\ \hline
% \textbf{INO (Ours)}               & -                            & Kinetics                                           & \textbf{71.3}                  & \textbf{70.7}   & \textbf{73.2}   & 65.6             & \textbf{75.6}    \\ \hline
% \end{tabular}


\begin{tabular}{l|cccccc}
\hline
\rowcolor{LightGray}
 &  &  & \multicolumn{2}{c}{\textbf{Seen}} & \multicolumn{2}{c}{\textbf{Unseen}} \\\cline{4-7}
\rowcolor{LightGray}
\multirow{-2}{*}{\textbf{Method}}   & \multirow{-2}{*}{\textbf{Dataset}}                               &   \multirow{-2}{*}{\textbf{Mean}}                            & \textbf{\Jm}     & \textbf{\Fm}     & \textbf{\Jm}      & \textbf{\Fm}      \\ \hline \hline
Colorize \cite{Colorize_vondrick2018tracking}                                         & Kinetics                                           & 38.9                           & 43.1            & 38.6            & 36.6             & 37.4             \\ 
CorrFlow\dag \cite{CorrFlow_lai2019self}                                        & OxUvA                                              & 46.6                           & 50.6            & 46.6            & 43.8             & 45.6             \\ 
MAST\dag \cite{MAST_lai2020mast}                                           & YT-VOS                                             & 64.2                           & 63.2            & 64.9            & 60.3             & 67.7             \\ 
CRW \cite{VRW_jabri2020space}                                         & Kinetics                                           & 69.9                           & 68.7            & 70.2            & 65.4             & 75.2             \\ 
DUL \cite{Dense_araslanov2021dense}                                            & YT-VOS                                           & 69.9                           & 69.6            & 71.3            & 65.0    & 73.5             \\
DUL \cite{Dense_araslanov2021dense}                                         & Kinetics                                           & 70.6                           & 69.9            & 71.3            & \textbf{66.5}    & 74.8             \\
DUL \cite{Dense_araslanov2021dense}                                        & TrackingNet                                        & 70.7                           & 70.2            & 71.9            & 66.3             & 74.5             \\ \hline
\textbf{INO (Ours)}                            & Kinetics                                           & \textbf{71.3}                  & \textbf{70.7}   & \textbf{73.2}   & 65.6             & \textbf{75.6}    \\ \hline
\end{tabular}
\end{center}
\label{table:YTVOS_with_SOTA}
\vspace{-4mm}
\end{table}


==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/table/efficiency.tex <==
\begin{table}[h]
% \footnotesize
\small
\caption{Comparison of efficiency when training on Kinetics-400.}
\vspace{-1mm}
\begin{center}
 \setlength{\tabcolsep}{3.9mm}{
\begin{tabular}{l|lccc}
\hline
\rowcolor{LightGray}
\textbf{Method} & \textbf{Arch} & \textbf{Param} & \textbf{GPUs}    & \textbf{Time} \\ \hline
VFS~\cite{Rethinking_xu2021rethinking}    & RN-50         & 23M              & $8 \times 24GB$ & 1week         \\ 
INO (ours)    & ViT-S/8       & 21M              & $8 \times 16GB$   & 1week         \\ \hline
\end{tabular}}
\end{center}
\label{table:efficiecy}
\vspace{-1mm}
\end{table}

==> [ACMMM22] 🍔In-N-Out Generative Learning for Dense Unsupervised Video Segmentation_camera_ready_final (1)/table/method-comparision.tex <==
% ===== No metgod version =====
% \begin{table}[t]
% % \footnotesize
% \tiny
% \caption{\textcolor{red}{Comparisons between different state-of-the-art VOS methods.}}
% \vspace{-2mm}
% % \renewcommand{\arraystretch}{1.1}
% \begin{center}
% {
% \setlength{\tabcolsep}{2.0mm}{
% \begin{tabular}{l|c|c|c|c|c}
% \rowcolor{LightGray}
% \hline
% Method &\makecell{Self-\\supervised} & \makecell{Transformer-\\ based} & \makecell{Pixel-level\\ Optimization} & \makecell{Image-level\\ Optimization} & \makecell{Generative \\learning} \\ \hline\hline
% CFBI (TPAMI 2021)~\cite{CFBI_yang2021collaborative} & \xmark & \xmark & \cmark &  \xmark & \xmark  \\ \hline
% CRW  (NIPS 2020)~\cite{VRW_jabri2020space} & \cmark & \xmark & \xmark & \cmark & \xmark \\ \hline
% VFS  (ICCV 2021)~\cite{Rethinking_xu2021rethinking} & \cmark & \xmark & \xmark & \cmark & \xmark \\ \hline
% DUL  (NIPS 2021)~\cite{Dense_araslanov2021dense} & \cmark & \xmark & \cmark & \xmark &  \xmark \\ \hline
% \textbf{INO (Ours)} & \cmark & \cmark & \cmark & \cmark &  \cmark \\
% \hline
% \end{tabular}}
% }
% \end{center}
% \label{table:method-comparision}
% \vspace{-5mm}
% \end{table}


% ===== text version ===== 
% \begin{table}[t]
% \footnotesize
% % \tiny
% \caption{Comparisons between different state-of-the-art VOS methods.}
% \vspace{-2mm}
% % \renewcommand{\arraystretch}{1.1}
% \begin{center}
% {
% \setlength{\tabcolsep}{1.3mm}{
% \begin{tabular}{l|c|c|c|c}
% \rowcolor{LightGray}
% \hline
% Method &\makecell{Self-\\supervised} & \makecell{CNN \\ vs. \\ ViT} & \makecell{Pixel \\ vs. \\ Image} &  \makecell{Contrastive \\ vs. \\ Generative} \\ \hline\hline
% CFBI (TPAMI 2021)~\cite{CFBI_yang2021collaborative} & \xmark & CNN & Pixel  & \xmark  \\ \hline
% CRW  (NIPS 2020)~\cite{VRW_jabri2020space}          & \cmark & CNN & Image      &  \xmark \\ \hline
% VFS  (ICCV 2021)~\cite{Rethinking_xu2021rethinking} & \cmark & CNN & Image      & \xmark \\ \hline
% DUL  (NIPS 2021)~\cite{Dense_araslanov2021dense}    & \cmark & CNN & Pixel       &  \xmark \\ \hline
% \textbf{INO (Ours)}                                 & \cmark & ViT & Pixel+Image &  \cmark \\
% \hline
% \end{tabular}}
% }
% \end{center}
% \label{table:method-comparision}
% \vspace{-5mm}
% \end{table}

% ====== original version =====
\begin{table}[t]
\footnotesize
% \tiny
\caption{Comparisons between different state-of-the-art VOS methods.}
\vspace{-2mm}
% \renewcommand{\arraystretch}{1.1}
\begin{center}
{
\setlength{\tabcolsep}{1.1mm}{
\begin{tabular}{l|c|c|c|c}
\rowcolor{LightGray}
\hline
Method &\makecell{Self-\\supervised} & \makecell{Transformer- \\ based} & \makecell{Unified \\optimization} &  \makecell{Generative \\learning} \\ \hline\hline
AOT (NIPS 2021)~\cite{yang2021associating} & \xmark & \cmark & \xmark & \xmark  \\ \hline
CRW  (NIPS 2020)~\cite{VRW_jabri2020space} & \cmark & \xmark & \xmark &  \xmark \\ \hline
VFS  (ICCV 2021)~\cite{Rethinking_xu2021rethinking} & \cmark & \xmark & \xmark & \xmark \\ \hline
DUL  (NIPS 2021)~\cite{Dense_araslanov2021dense} & \cmark & \xmark & \xmark &  \xmark \\ \hline
\textbf{INO (Ours)} & \cmark & \cmark & \cmark &  \cmark \\
\hline
\end{tabular}}
}
\end{center}
\label{table:method-comparision}
\vspace{-5mm}
\end{table}

==> figure/DAVIS_badcase.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figure/DAVIS_badcase.pdf}
% \DeclaregraphicsExtensions
\vspace{-4mm}
\caption{\textbf{Failure cases on DAVIS-2017 \texttt{val}.} 
}
% \vspace{-3mm}
\label{fig_DAVIS_badcase}
\end{figure*}


==> figure/YTVOS_badcase.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{./figure/YTVOS_badcase.pdf}
% \DeclaregraphicsExtensions
\vspace{-4mm}
\caption{\textbf{Failure cases on YouTube-VOS 2018 \texttt{val}.} 
}
\vspace{-3mm}
\label{fig_YTVOS_badcase}
\end{figure*}


==> figure/intro.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=4.8in]{./figure/intro.pdf}
\DeclaregraphicsExtensions
\caption{ \textbf{}  }
\label{fig_intro}
\end{figure}

